Machine Learning and Deep Learning methods for predictive modelling from Raman spectra in bioprocessing

In chemical processing and bioprocessing, conventional online sensors are limited to measure only basic process variables like pressure and temperature, pH, dissolved O and CO$_2$ and viable cell density (VCD). The concentration of other chemical species is more difficult to measure, as it usually requires an at-line or off-line approach. Such approaches are invasive and slow compared to on-line sensing. It is known that different molecules can be distinguished by their interaction with monochromatic light, producing different profiles for the resulting Raman spectrum, depending on the concentration. Given the availability of reference measurements for the target variable, regression methods can be used to model the relationship between the profile of the Raman spectra and the concentration of the analyte. This work focused on pretreatment methods of Raman spectra for the facilitation of the regression task using Machine Learning and Deep Learning methods, as well as the development of new regression models based on these methods. In the majority of cases, this allowed to outperform conventional Raman models in terms of prediction error and prediction robustness.

==> chapters/preamble.tex <==
%---------------------------------------------------------------------------
% Preface

% \chapter*{Preface}

% Blah blah \dots

%  \cleardoublepage

%---------------------------------------------------------------------------
% Table of contents

 \setcounter{tocdepth}{2}
 \tableofcontents

 \cleardoublepage

%---------------------------------------------------------------------------
% Abstract

% \chapter*{Zusammenfassung}
%  \addcontentsline{toc}{chapter}{Zusammenfassung}

%  \cleardoublepage

\chapter*{Abstract}
 \addcontentsline{toc}{chapter}{Abstract}

 \cleardoublepage

%---------------------------------------------------------------------------
% Symbols

% \chapter*{Nomenclature}\label{chap:symbole}
%  \addcontentsline{toc}{chapter}{Nomenclature}

% \section*{Symbols}
% \begin{tabbing}
%  \hspace*{1.6cm} \= \hspace*{8cm} \= \kill
%  $\mathrm{EHC}$ \> Conditional equation \> [$-$] \\[0.5ex]
%  $e$ \> Willans coefficient \> [$-$] \\[0.5ex]
%  $F,G$ \> Parts of the system equation \> [\unitfrac[]{K}{s}]
% \end{tabbing}

% \section*{Indicies}
% \begin{tabbing}
%  \hspace*{1.6cm}  \= \kill
%  a \> Ambient \\[0.5ex]
%  air \> Air
% \end{tabbing}

% \section*{Acronyms and Abbreviations}
% \begin{tabbing}
%  \hspace*{1.6cm}  \= \kill
%  NEDC \> New European Driving Cycle \\[0.5ex]
%  ETH \> Eidgen\"{o}ssische Technische Hochschule
% \end{tabbing}

%  \cleardoublepage

%---------------------------------------------------------------------------


==> chapters/pythonscripts.tex <==


\begin{figure}[h]
  \begin{minipage}[h]{0.98\textwidth}
    \begin{lstlisting}[language=Python, caption=Python implementation of used shuffling algorithm]
    def skip_grouper(n, iterable):
        i = 0
        len_it = math.ceil(len(iterable) / n)
        while i < len_it:
            chunk = iterable[i::len_it]
            i += 1
            yield chunk
            
    \end{lstlisting}
    \end{minipage}
    \label{alg:skipgrouper}
\end{figure}


\begin{figure}[h]
  \begin{minipage}[h]{0.98\textwidth}
    \begin{lstlisting}[language=Python, caption=Python code for data augmentation]

def augment_data(x: np.ndarray, offset=0.05, multi=0.05, noise=0.001, cumulative_noise=0.001):
    offset_range = offset * np.std(x, 0)
    multishift = multi
    noise_range = noise * np.std(x, 0)
    cum_noise_range = cumulative_noise * np.std(x, 0)

    x = x + np.random.random(size=x.shape) * 2 * offset_range - offset_range
    x = x * (np.random.random(size=x.shape) * 2 * multishift - multishift + 1)
    x = x + np.random.random(size=x.shape) * noise_range * 2 - noise_range
    x = x + np.cumsum(np.random.random(size=x.shape) * cum_noise_range * 2 - cum_noise_range, axis=0)

    return x
    \end{lstlisting}
    \label{pythonaugmentation}
    \end{minipage}
\end{figure}



\begin{figure}[h]
  \begin{minipage}[h]{0.98\textwidth}
    \begin{lstlisting}[language=Python, caption=Python code for data augmentation and resampling]

def apply_custom_data_augmentation(x_original: np.ndarray, y_original: np.ndarray,
    ratio=0.1, binsize=0.5, counts_min=None, decay=None, normal=False,
    offset=0.001, multi=0.0005, noise=0.0005, cumulative_noise=0.001):
    
    features = x_original
    targets = y_original
    mean = y_original.mean()
    std = y_original.std()
    
    # if min number of samples per bin is required
    if counts_min:
        bins = np.arange(np.floor(y_original.min()), np.ceil(y_original.max() + binsize), binsize)
        counts, binEdges = np.histogram(y_original, bins=bins)
        # augment bin size if necessary
        while counts.min() < counts_min:
            binsize += binsize * 0.1
            bins = np.arange(np.floor(y_original.min()), np.ceil(y_original.max() + binsize), binsize)
            counts, binEdges = np.histogram(y_original, bins=bins)
    else:
        bins = np.arange(np.floor(y_original.min()), np.ceil(y_original.max() + binsize), binsize)
        counts, binEdges = np.histogram(y_original, bins=bins)

    binIdx = np.digitize(y_original, binEdges)

    if normal:
        # prepare normal distribution
        gauss = np.random.normal(mean, std, int(len(targets) * (1 + ratio)))
        gauss += gauss.max() * 0.1
        counts_g, _ = np.histogram(gauss, bins=bins)
        counts_g += int(counts_g.max()*0.1)


    counts_max = counts.max()
    counts_tar = int(ratio * counts_max)

    binIdx_lst = list(set(binIdx))
    # for every bin :
    for idx in binIdx_lst:
        # find indices of x and y for current bin
        indices_bin = np.where(binIdx == idx)
        bins_y = y_original[indices_bin]
        bins_x = x_original[indices_bin]
        # while current bin's count below target
        if decay:
            counts_tar = round(counts_tar * decay)
            ratio_bin = counts[idx - 1] / counts_tar
        elif normal:
            counts_tar = counts_g[idx - 1]
            ratio_bin = counts[idx - 1] / counts_tar
        else:
            ratio_bin = counts[idx - 1] / counts_tar
        ratio_aug_bin = 1.0 / ratio_bin

        if counts[idx - 1] < counts_tar:
            # chose random index from current bin n times
            sample_n = counts_tar - counts[idx - 1]
            sampled_bin_idx = np.random.choice(np.arange(len(bins_y)), sample_n)
            features = np.vstack(
                (features, augment_data(bins_x[sampled_bin_idx],
                offset, multi, noise, cumulative_noise)))
            targets = np.hstack((targets, bins_y[sampled_bin_idx]))
    return features, targets
    \end{lstlisting}
        \label{pythonresampling}
    \end{minipage}
\end{figure}






\begin{figure}[!h]
  \begin{minipage}[h]{0.98\textwidth}
    \begin{lstlisting}[language=Python, caption=Python code for Ranking Feature Importance based on XGB]

from ramanModules.dataLoading import load_dataset, load_var_dataset
from ramanModules.RamanConstants import name2var, var2Name, possible_dataset_ids, var2Unit, processed_data_path
from ramanModules.Modeling import prepare_data, get_batch_list_with_var, get_preprocessing_pipeline
import argparse
import pandas as pd
import numpy as np
import xgboost
import pprint as pp
import os
import plotly
import plotly.graph_objs as go
from plotly.offline import download_plotlyjs, init_notebook_mode, iplot, plot

def main():
    parser = argparse.ArgumentParser()
    parser.add_argument('--var', choices=name2var.keys(), default='Titer')
    parser.add_argument(
        '--dataset',
        choices=possible_dataset_ids,
        default=None
    )
    parser.add_argument(
        '--test_p',
        default = None
    )
    parser.add_argument(
        '--test_l',
        default = 1
    )
    parser.add_argument(
        '--datasets',
        nargs='*',
        default=None
    )
    parser.add_argument(
        '--n_estimators',
        default=1000
    )
    parser.add_argument(
        '--max_depth',
        default=6
    )
    parser.add_argument(
        '--learning_rate',
        default=0.01
    )
    parser.add_argument(
        '--top',
        default=100
    )
    parser.add_argument(
        '--reload',
        default=True
    )


    args = parser.parse_args()
    dataset_id = args.dataset
    learning_rate = float(args.learning_rate)
    n_estimators = int(args.n_estimators)
    max_depth = int(args.max_depth)
    top = int(args.top)
    var_name = args.var
    path = str(processed_data_path) + "/feature_importance_{}_{}".format(dataset_id, var_name)
    print('path : ', path)
    target, spectrum = load_dataset(processed_data_path=processed_data_path, dataset_id=args.dataset)
    spect, tar = prepare_data(spectrum, target, name2var[args.var])
    preprocessing_pipeline = get_preprocessing_pipeline(spect.columns, window_length=17, polyorder=2, deriv=1, dropcols='standard')
    
    col_names_pp = list(range(450, 1821)) + list(range(1880, 2531)) + list(
        range(2590, 3101))
    spect = pd.DataFrame(
        preprocessing_pipeline.fit_transform(spect.values),
        index=spect.index,
        # invalid key error:
        columns=col_names_pp)

    if args.reload == 'True' and os.path.exists(path + '.csv'):
        print('reloading feature_importance...')
        feature_importance = pd.read_csv(path + '.csv')
    else:
        print('calculating feature_importance...')
        xgb = xgboost.XGBRegressor(nthread=-1, n_estimators=n_estimators, learning_rate=learning_rate, gamma=0, subsample=0.75,
                                   colsample_bytree=1, max_depth=max_depth)
        xgb.fit(spect, tar)
        # feature_importance = pd.DataFrame(list(zip(range(len(xgb.feature_importances_)), xgb.feature_importances_)),
        # pass column names
        feature_importance = pd.DataFrame(list(zip(range(len(xgb.feature_importances_)), col_names_pp, xgb.feature_importances_)),

                                          columns=['col_ind', 'col_name', 'feature_importance_vals'])
        feature_importance.sort_values(by=['feature_importance_vals'], ascending=False, inplace=True)
        feature_importance.to_csv(path + '.csv')

        fig = go.Figure(
            data=[go.Bar(x=feature_importance['col_name'], y=feature_importance['feature_importance_vals'])])
        plotly.offline.plot(fig, filename=path + '.html', auto_open=False)

    selected_features = feature_importance.head(top)

    print('len(selected_features) : ', len(selected_features))

    fig = go.Figure(
        data=[go.Bar(x=selected_features['col_name'], y=selected_features['feature_importance_vals'])])
    plotly.offline.plot(fig, filename=path + '_top_' + str(top) + '.html', auto_open=False)

    # cols_to_drop = sorted(set(spect.columns.values).difference(set(selected_features['col_name'].values)))
    # drop by index and not by name :
    cols_to_drop = sorted(set(range(spect.shape[1])).difference(set(selected_features['col_ind'].values)))

    # cols_to_drop are sorted, so the dropped df is also sorted, but selected_features['col_name'] are not...

    # col_names need to be sorted!
    col_names = sorted(selected_features['col_name'] )
    np.savetxt(processed_data_path / 'important_cols_{}_{}_top_{}.txt'.format(dataset_id, var_name, top),col_names, fmt='%d')
    np.savetxt(processed_data_path / 'cols_to_drop_{}_{}_top_{}.txt'.format(dataset_id, var_name, top), cols_to_drop, fmt='%d')


if __name__ == '__main__':
    main()

    \end{lstlisting}
        \label{pythonfeatureimportance}
    \end{minipage}
\end{figure}



==> chapters/results.tex <==



==> tables/13_all_Titer_XGB-GP-SVR-PLS_STD-AUG-RES.tex <==
\begin{table}[h!]%
\caption{ML models N RMSE comparison for (STD, STD+AUG, STD+RES) on DS1 Titer}%
\renewcommand*{\MinNumber}{0.191}%
\renewcommand*{\MidNumber}{0.259}%
\renewcommand*{\MaxNumber}{0.37200000000000005}%
\centering%
\begin{adjustbox}{width=0.98\textwidth}%
\begin{tabular}{@{}lR@{\hskip-1.5\tabcolsep}R@{\hskip-1.5\tabcolsep}RR@{\hskip-1.5\tabcolsep}R@{\hskip-1.5\tabcolsep}RR@{\hskip-1.5\tabcolsep}R@{\hskip-1.5\tabcolsep}RR@{\hskip-1.5\tabcolsep}R@{\hskip-1.5\tabcolsep}RR@{\hskip-1.5\tabcolsep}R@{\hskip-1.5\tabcolsep}R@{}}%
\toprule%
\multirow{2}{*}{TEST BATCHES}&\multicolumn{3}{c}{XGB}&\multicolumn{3}{c}{GP}&\multicolumn{3}{c}{SVR}&\multicolumn{3}{c}{PLS}&\multicolumn{3}{c}{Benchmark}\\%
&STD&AUG&RES&STD&AUG&RES&STD&AUG&RES&STD&AUG&RES&STD&AUG&RES\\%
\midrule%
\EndTableHeader%
1,7,52,67,97,103,117,127&0.306&0.282&0.317&0.257&0.332&0.296&0.359&0.387&0.384&0.229&0.273&0.238&0.229&0.273&0.238\\%
2,8,53,92,98,104,118&0.284&0.289&0.294&0.256&0.291&0.302&0.328&0.302&0.319&0.294&0.339&0.320&0.294&0.339&0.320\\%
3,9,54,93,99,105,119&0.309&0.333&0.312&0.277&0.331&0.352&0.405&0.413&0.390&0.210&0.251&0.228&0.210&0.251&0.228\\%
4,10,55,94,100,106,124&0.139&0.181&0.158&0.128&0.195&0.231&0.195&0.269&0.252&0.191&0.193&0.215&0.191&0.193&0.215\\%
5,38,65,95,101,107,125&0.313&0.302&0.315&0.271&0.322&0.304&0.395&0.341&0.367&0.272&0.367&0.347&0.272&0.367&0.347\\%
6,39,66,96,102,116,126&0.447&0.466&0.455&0.407&0.438&0.412&0.487&0.503&0.506&0.372&0.410&0.380&0.372&0.410&0.380\\%
AVG BATCHES&0.300&0.309&0.308&0.266&0.318&0.316&0.361&0.369&0.369&0.261&0.306&0.288&0.261&0.306&0.288\\%
AVG OVERALL&0.309&0.317&0.316&0.274&0.324&0.321&0.370&0.379&0.376&0.259&0.303&0.283&0.259&0.303&0.283\\\bottomrule%
%
\end{tabular}%
\end{adjustbox}%
\label{tab:DS13_ML_Titer_AUG}
\end{table}
